Spectral Maps for Learning on Subgraphs

In graph learning, maps between graphs and their subgraphs frequently arise. For instance, when coarsening or rewiring operations are present along the pipeline, one needs to keep track of the corresponding nodes between the original and modified graphs. Classically, these maps are represented as binary node-to-node correspondence matrices and used as-is to transfer node-wise features between the graphs. In this paper, we argue that simply changing this map representation can bring notable benefits to graph learning tasks. Drawing inspiration from recent progress in geometry processing, we introduce a spectral representation for maps that is easy to integrate into existing graph learning models. This spectral representation is a compact and straightforward plug-in replacement and is robust to topological changes of the graphs. Remarkably, the representation exhibits structural properties that make it interpretable, drawing an analogy with recent results on smooth manifolds. We demonstrate the benefits of incorporating spectral maps in graph learning pipelines, addressing scenarios where a node-to-node map is not well defined, or in the absence of exact isomorphism. Our approach bears practical benefits in knowledge distillation and hierarchical learning, where we show comparable or improved performance at a fraction of the computational cost.

==> figures/onlyrewire_inc.tex <==
\begin{figure}[t]
\vspace{0.2cm}
\centering
\begin{overpic}
[trim=0cm 0cm 0cm 0cm,clip,width=0.999\linewidth, grid=false]{./figures/onlyrewiring_C.png}
%
\put(2,34){\tiny Minnesota}
\put(4,23){\tiny CORA}
\put(4,9){\tiny Karate}
%
\put(100,31){\tiny $1$}
\put(100,25){\tiny $\scalebox{0.7}[1.0]{-}1$}
%
\put(14.5,32){\tiny $8\%$}
\put(22.5,32){\tiny $16\%$}
\put(31.5,32){\tiny $24\%$}
\put(40,32){\tiny $32\%$}
\put(49,32){\tiny $40\%$}
\put(57.5,32){\tiny $48\%$}
\put(66.5,32){\tiny $56\%$}
\put(75.5,32){\tiny $64\%$}
\put(84,32){\tiny $72\%$}
\put(92.5,32){\tiny $80\%$}
%
\put(14.5,19.7){\tiny $8\%$}
\put(22.5,19.7){\tiny $16\%$}
\put(31.5,19.7){\tiny $24\%$}
\put(40,19.7){\tiny $32\%$}
\put(49,19.7){\tiny $40\%$}
\put(57.5,19.7){\tiny $48\%$}
\put(66.5,19.7){\tiny $56\%$}
\put(75.5,19.7){\tiny $64\%$}
\put(84,19.7){\tiny $72\%$}
\put(92.5,19.7){\tiny $80\%$}
%
\put(14.5,7.7){\tiny $8\%$}
\put(22.5,7.7){\tiny $16\%$}
\put(31.5,7.7){\tiny $24\%$}
\put(40,7.7){\tiny $32\%$}
\put(49,7.7){\tiny $40\%$}
\put(57.5,7.7){\tiny $48\%$}
\put(66.5,7.7){\tiny $56\%$}
\put(75.5,7.7){\tiny $64\%$}
\put(84,7.7){\tiny $72\%$}
\put(92.5,7.7){\tiny $80\%$}
\end{overpic}
\caption{\label{fig:graphsOnlyRewiringInc} Robustness of the map to rewiring of the subgraph.
The rewiring operations are increasingly stronger, with increments of 8\% of the total number of
edges (starting from 8\% and reaching 80\%). The plotted matrices represent the functional map after the topological perturbations, showing the effect
of rewiring on the functional map structure.}
\end{figure}

==> figures/onlyrewire_wider.tex <==
\begin{figure}[t]
\vspace{0.2cm}
\centering
\begin{overpic}
[trim=0cm 0cm 0cm 0cm,clip,width=0.999\linewidth, grid=false]{./figures/onlyrewiring_Widerpsd.png}
%
\put(5,40){\tiny cat}
\put(3,28.5){\tiny Minnesota}
\put(5,15){\tiny CORA}
%
\put(100,41){\tiny $1$}
\put(100,32.5){\tiny $\scalebox{0.7}[1.0]{-}1$}
%
\put(19,43.5){\tiny $1\%$}
\put(33,43.5){\tiny $5\%$}
\put(47.5,43.5){\tiny $10\%$}
\put(61.5,43.5){\tiny $30\%$}
\put(76,43.5){\tiny $50\%$}
\put(90,43.5){\tiny $100\%$}
%
\put(19,28.5){\tiny $1\%$}
\put(33,28.5){\tiny $5\%$}
\put(47.5,28.5){\tiny $10\%$}
\put(61.5,28.5){\tiny $30\%$}
\put(76,28.5){\tiny $50\%$}
\put(90,28.5){\tiny $100\%$}
%
\put(19,13.5){\tiny $1\%$}
\put(33,13.5){\tiny $5\%$}
\put(47.5,13.5){\tiny $10\%$}
\put(61.5,13.5){\tiny $30\%$}
\put(76,13.5){\tiny $50\%$}
\put(90,13.5){\tiny $100\%$}
\end{overpic}
\caption{\label{fig:graphsOnlyRewiringWider} Robustness of the map to rewiring of the subgraph.
The rewiring operations are increasingly wider, involving nodes and edges farther apart. The left
column shows the full graph, while the others columns show the resulting functional map, starting with a rewiring involving just nodes within 1\% of
the graph diameter (left) up to the full graph diameter (right)}
\end{figure}

==> sections/Figs/sigtransf_fig.tex <==
\begin{figure}[h]
\caption{Normalized Mean Squared Error (MSE) obtained by transferring node features using the functional map on a truncated eigenbasis (50 eigenfunctions).}
\begin{minipage}[c]{0.4\linewidth}
\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{l|cccc}
Dataset & Task & Type & Subgraph & Features \\ \hline
        Citeseer & 2120 & citation & class & continuous and sparse  \\ 
        PubMed & 19717 & citation & class & continuous and sparse \\ 
        PPI 0 & 1546 & molecular & label & continuous  \\ 
        PPI 13 & 3480 & molecular & label & continuous  \\ 
        FraudAmazon & 11944 & reviews & edge type & mixed \\ 

        Amazon Photo & 7487 &  co-purchase & class & discrete and sparse  \\ 
        Amazon Computer & 13381 & co-purchase & class & discrete and sparse \\ 
\end{tabular}
\label{tab:func_transfer}
\end{table}
\end{minipage}
\begin{minipage}[c]{0.4\linewidth}
\centering
\begin{overpic}
[clip,width=0.65\linewidth,grid=False]{./figures/NRMSE_mean.png}
\put(34,0){Percentage of eigenvectors}
\put(0,29){\rotatebox[origin=c]{90}{Mean Squared Error}}
\end{overpic}
\caption{Mean Squared Error (MSE) obtained by transferring node features, using a functional map with increasing number of eigenfunctions (expressed as a percentage).}
\label{fig:transfer_error_vs_k}
\end{minipage}
\end{figure}

==> sections/Tabels/TAB_cat0.4patch.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|l|l|l|l|l|l|l}
         & accuracy & MAP      & AUC      & Hit      & precision\_5 & precision\_10 & time     \\ \hline
IsoRank  & 0.00               & 0.00 & 0.50 & 0.50 & 0.00         & 0.00          & 266.15  \\ \hline
BigAlign & 0.51               & 0.02 & 0.92 & 0.92 & 0.01         & 0.03          & 0.58    \\ \hline
FINAL    & 0.01               & 0.00 & 0.58 & 0.58 & 0.00         & 0.00          & 183.54  \\ \hline
REGAL    & 0.91               & 0.93 & 1.00 & 1.00 & 0.98         & 0.99          & 37.35   \\ \hline \hline
fmW      & 0.62               & 0.69 & 1.00 & 1.00 & 0.75         & 0.81          & 95.60   \\ \hline
fmW\_ZM  & 0.64               & 0.70 & 1.00 & 1.00 & 0.75         & 0.81          & 70.94   \\ \hline
GRASP & 0.11 & 0.11 & 0.96 & 0.96 & 0.16 & 0.28 & 1053.72 \\ \hline
gt       & 0.85               & 0.92 & 1.00 & 1.00 & 0.97         & 0.99          & 61.44   \\ \hline \hline
PALE     & 0.97               & 0.95 & 1.00 & 1.00 & 1.00         & 1.00          & 3869.36 \\ \hline
\end{tabular}
\caption{Cat 0.4 patch}
\label{tab:cat0.4patch}
\end{table}

==> sections/Tabels/TAB_cat0.4patchmesh.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|l|l|l|l|l|l|l}
         & accuracy & MAP      & AUC      & Hit      & precision\_5 & precision\_10 & time     \\ \hline
IsoRank & 0.00 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 270.44 \\ \hline
BigAlign & 0.49 & 0.02 & 0.92 & 0.92 & 0.01 & 0.03 & 0.55 \\ \hline
FINAL & 0.01 & 0.00 & 0.58 & 0.58 & 0.00 & 0.00 & 156.49 \\ \hline
REGAL & 0.91 & 0.93 & 1.00 & 1.00 & 0.97 & 0.99 & 36.78 \\  \hline \hline
fmW & 0.61 & 0.68 & 1.00 & 1.00 & 0.73 & 0.80 & 79.56 \\ \hline
fmW\_ZM & 0.63 & 0.69 & 1.00 & 1.00 & 0.74 & 0.80 & 64.28 \\ \hline
GRASP & 0.12 & 0.11 & 0.96 & 0.96 & 0.16 & 0.28 & 1057.74 \\ \hline
gt & 0.85 & 0.92 & 1.00 & 1.00 & 0.98 & 0.99 & 58.83 \\ \hline \hline
fmW\_neum & 0.01 & 0.05 & 0.91 & 0.91 & 0.07 & 0.12 & 21.33 \\ \hline
gt\_neum & 0.22 & 0.39 & 1.00 & 1.00 & 0.58 & 0.70 & 2.97 \\ \hline
\end{tabular}
\caption{Cat 0.4 patch\_mesh}
\label{tab:Cat0.4patch_mesh}
\end{table}

==> sections/Tabels/TAB_cora0.4patch.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|l|l|l|l|l|l|l}
         & accuracy & MAP      & AUC      & Hit      & precision\_5 & precision\_10 & time     \\ \hline
IsoRank  & 0.01               & 0.01 & 0.51 & 0.51 & 0.00         & 0.01          & 31.54  \\ \hline
BigAlign & 0.29               & 0.04 & 0.90 & 0.90 & 0.04         & 0.08          & 0.03   \\ \hline
FINAL    & 0.04               & 0.01 & 0.55 & 0.55 & 0.00         & 0.01          & 10.48  \\ \hline
REGAL    & 0.45               & 0.54 & 0.99 & 0.99 & 0.64         & 0.74          & 7.33   \\ \hline \hline
fmW      & 0.20               & 0.33 & 0.96 & 0.96 & 0.42         & 0.52          & 4.12   \\ \hline
fmW+ZM  & 0.21               & 0.34 & 0.96 & 0.96 & 0.43         & 0.53          & 1.62   \\ \hline
GRASP & 0.15 & 0.07 & 0.71 & 0.72 & 0.09 & 0.14 & 198.22\\ \hline
gt       & 0.53               & 0.65 & 1.00 & 1.00 & 0.78         & 0.86          & 1.23   \\ \hline  \hline
PALE     & 0.77               & 0.72 & 1.00 & 1.00 & 0.88         & 0.95          & 435.43 \\ \hline
\end{tabular}
\caption{CORA 0.4 patch}
\label{tab:CORA0.4patch}
\end{table}

==> sections/Tabels/TAB_cora1.0class.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|l|l|l|l|l|l|l}

         & accuracy & MAP  & AUC  & Hit  & precision\_5 & precision\_10 & time    \\ \hline
IsoRank  & 0.01  $\pm$ 0.00             & 0.00 & 0.51 & 0.51 & 0.00         & 0.00          & 14.92   \\ \hline
BigAlign & 0.43 $\pm$ 0.14 & 0.03 & 0.90 & 0.90 & 0.03         & 0.07          & 0.22    \\ \hline
FINAL    & 0.10  $\pm$ 0.06 & 0.00 & 0.55 & 0.55 & 0.00         & 0.01          & 51.61   \\ \hline
REGAL    & 0.46 $\pm$ 0.04 & 0.55 & 1.00 & 1.00 & 0.65         & 0.74          & 10.92   \\ \hline \hline
fmW      & 0.60     $\pm$ 0.2          & 0.71 & 0.97 & 0.97 & 0.82         & 0.87          & 3.42    \\ \hline
fmW\_ZM  & 0.47  $\pm$ 0.24 & 0.60 & 0.97 & 0.97 & 0.71         & 0.79          & 1.84    \\ \hline
GrASP    & 0.60  $\pm$ 0.18 & 0.51 & 0.94 & 0.94 & 0.64         & 0.72          & 118.61  \\ \hline
gt       & 0.78 $\pm$ 0.09 & 0.85 & 1.00 & 1.00 & 0.94         & 0.97          & 1.46    \\ \hline \hline
PALE     & 0.83 $\pm$ 0.02 & 0.72 & 1.00 & 1.00 & 0.89         & 0.96          & 1056.03 \\ \hline
\end{tabular}
\caption{Cora where the partiality is obtained removing one class(according to the labels on the nodes) at the time. This is similar to removing a cluster of nodes.}
\label{tab:cora1class}
\end{table}

==> sections/Tabels/TAB_douban.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|l|l|l|l|l|l|l}
         & accuracy & MAP      & AUC      & Hit      & precision\_5 & precision\_10 & time     \\ \hline
IsoRank  & 0.00               & 0.01 & 0.50 & 0.50 & 0.00         & 0.01          & 11.54   \\ \hline
BigAlign & 0.03               & 0.02 & 0.76 & 0.76 & 0.02         & 0.05          & 0.14    \\ \hline
FINAL    & 0.02               & 0.01 & 0.56 & 0.56 & 0.01         & 0.01          & 27.07   \\ \hline
REGAL    & 0.56               & 0.70 & 1.00 & 1.00 & 0.79         & 0.89          & 10.41   \\ \hline \hline
fmW      & 0.00               & 0.01 & 0.51 & 0.51 & 0.01         & 0.01          & 8.80    \\ \hline
fmW\_ZM  & 0.00               & 0.01 & 0.52 & 0.52 & 0.01         & 0.01          & 4.44    \\ \hline
GRASP    & 0.00               & 0.01 & 0.51 & 0.51 & 0.00         & 0.01          & 16.32   \\ \hline
gt       & 0.00               & 0.03 & 0.63 & 0.63 & 0.04         & 0.07          & 4.37    \\ \hline \hline
PALE     & 0.19               & 0.21 & 0.64 & 0.64 & 0.22         & 0.24          & 1145.63 \\ \hline
\end{tabular}
\caption{Douban}
\label{tab:douban}
\end{table}

==> sections/Tabels/TAB_isomorph.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|l|l|l|l|l|l|l}
         & accuracy & MAP      & AUC      & Hit      & precision\_5 & precision\_10 & time     \\ \hline
IsoRank & 1.00 & 0.00 & 0.52 & 0.52 & 0.00 & 0.00 & 70.51 \\ \hline
 REGAL & 0.59 & 0.65 & 1.00 & 1.00 & 0.73 & 0.80 & 19.02 \\ \hline \hline
fmW\_ZM & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 7.54 \\ \hline
gt & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 5.99 \\ \hline
fmW & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 9.48 \\ \hline \hline
PALE & \\ \hline
\end{tabular}
\caption{Isomorphism test on random graph}
\label{tab:isomorph}
\end{table}

==> sections/Tabels/TAB_k_increase.tex <==
% MSE
% \begin{table}[h]
% \centering
% \caption{Normalized Mean Squared Error (MSE) obtained by transferring node features using the functional map on a truncated eigenbasis with increasing number of eigenfunctions.}
% \setlength{\tabcolsep}{1.1pt}
% \centering
% \tiny
% \begin{tabular}{l|ccccc| cccccc}
%  & \multicolumn{5}{c}{number of eigenvectors } & \multicolumn{6}{c}{percentage of eigenvectors } \\ 
% Dataset & 50 & 100 & 200 & 500 & 1000 & 10\% & 20\% & 30\% & 50\% & 75\% & 100\% \\ \hline
% PPI~\cite{PPI} 0 & & $\pm$ & $\pm$ & $\pm$ &$\pm$ & $0.02; std:0.0$ & $\pm$ & $0.02; std:0.0$ & $0.01; std:0.0$ & $0.01; std:0.0$ & $0.0; std:0.0$ \\ 
% PPI~\cite{PPI} 13 & & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $0.02; std:0.0$ & $\pm$ & $0.02; std:0.0$ & $0.01; std:0.0$ & $0.01; std:0.0$ & $0.0\pm0.0$ \\ \hline
% FraudAmazon~\cite{AmazonFraud} & & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\ \hline

% Amazon Photo~\cite{AmazonCoBuy} &  $18\pm2$ &$18\pm2$ & $17\pm2$ & $16\pm1$ & $15\pm1$ & $0.16\pm0.02$ & $0.14\pm0.01$ & $0.13\pm0.01$ & $0.10\pm0.01$ & $0.06\pm0.01$ & $0.0\pm0.0$ \\ 
% Amazon Computer~\cite{AmazonCoBuy} & $21\pm2$ & $20\pm2$  & $19\pm1$ & $18\pm0$ & $17\pm1$ & $0.18\pm0.01$ & $\pm$ & $0\pm0.$ & $0.11\pm0.01$ & & $0.00\pm0.00$ \\ 
% \end{tabular}
% \label{tab:MSE_FTransf_eigen}
% \end{table}

% Squared Relative Error
% \begin{table}[h]
% \centering
% \caption{Squared Relative Error obtained by transferring node features using the functional map on a truncated eigenbasis with increasing number of eigenfunctions.}
% \setlength{\tabcolsep}{1.1pt}
% \centering
% \tiny
% \begin{tabular}{l|ccccc| cccccc}
%  & \multicolumn{5}{c}{number of eigenvectors } & \multicolumn{6}{c}{percentage of eigenvectors } \\ 
% Dataset & 50 & 100 & 200 & 500 & 1000 & 10\% & 20\% & 30\% & 50\% & 75\% & 100\%\\ \hline
% PPI~\cite{PPI} 0 & & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\ 
% PPI~\cite{PPI} 13 & & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\ \hline
% FraudAmazon~\cite{AmazonFraud} & & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\ \hline

% Amazon Photo~\cite{AmazonCoBuy} &  & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $210.61\pm17.65$ & $190.97\pm17.39$ & $173.90\pm17.74$ & $137.74\pm17.39$ & $83.45\pm10.37$ & $2.69\pm4.24$ \\ 
% Amazon Computer~\cite{AmazonCoBuy} &  & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $1105.64\pm132.21$ & $\pm$ & $900.05\pm96.71$ & $706.50\pm77.64$ & $\pm$ & $20.42\pm40.52$\\ 
% \end{tabular}
% \label{tab:RE_FTransf_eigen}
% \end{table}

% % Absolute Relative Error
% \begin{table}[h]
% \centering
% \caption{Absolute Relative Error obtained by transferring node features using the functional map on a truncated eigenbasis with increasing number of eigenfunctions.}
% \setlength{\tabcolsep}{1.5pt}
% \centering
% \tiny
% \begin{tabular}{l|ccccc| cccccc}
%  & \multicolumn{5}{c}{number of eigenvectors } & \multicolumn{6}{c}{percentage of eigenvectors } \\ 
% Dataset & 50 & 100 & 200 & 500 & 1000 & 10\% & 20\% & 30\% & 50\% & 75\% & 100\%\\ \hline
% PPI~\cite{PPI} 0 & & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\ 
% PPI~\cite{PPI} 13 & & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\ \hline
% FraudAmazon~\cite{AmazonFraud} & & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\ \hline

% Amazon Photo~\cite{AmazonCoBuy} &  & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $2.80\pm0.22$ & $2.63\pm0.22$ & $2.48\pm0.21$ & $2.19\pm0.2$ & $1.69\pm0.12$ & $0.14\pm0.25$ \\ 
% Amazon Computer~\cite{AmazonCoBuy} &  & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $4.63\pm0.30$ & $\pm$ & $3.98\pm0.24$ & $3.46\pm0.22$ & & $0.19\pm0.37$ \\ 
% \end{tabular}
% \label{tab:REAbs_FTransf_eigen}
% \end{table}

==> sections/Tabels/TAB_laplace.tex <==
\begin{table}[h]
% \hspace{-2.4cm}
\setlength{\tabcolsep}{1.1pt}
\centering
\tiny
\caption{Comparison of the Mean Average Precision of the correspondence computed on different graphs by different methods. All the values are expressed as percentage.}
\begin{tabular}{l| C{0.8cm} | c c c | c c c | c c c| c c c}
% \begin{tabularx}{\textwidth}{l| C{0.8cm} | c c c | c c c | c c c| c c c}
 & Partiality & \multicolumn{3}{c}{Neumann mesh} & \multicolumn{3}{c}{Dirichlet mesh} & \multicolumn{3}{c}{graph}  & \multicolumn{3}{c}{normalized graph} \\
 & & FM$_{W}$ & FM$_{W}+$ZM & $GT$ & FM$_{W}$ & FM$_{W}+$ZM & $GT$  & FM$_{W}$ & FM$_{W}+$ZM & $GT$ & FM$_{W}$ & FM$_{W}+$ZM & $GT$ \\ \hline
Cat~\cite{shrec2016} & \multirow{3}{*}{patch}  & $5\pm1.4$ &  $2\pm0.5$  & $39\pm3$ & $8\pm4$ &  $0\pm0.2$  & $11\pm8.2$  & $11\pm3.3$ &  $40\pm22$  & $\textbf{92}\pm4.2$ & $68\pm14$ & $69\pm14$  & $\textbf{92}\pm3.9$ \\ 
Minnesota & - & - & - & - & - & - & - & $30\pm4.5$ &  $78\pm0.4$  & $92\pm0.0$  &   $88\pm4$ & $89\pm3.7$  & \textbf{$\textbf{94}\pm1.6$} \\
Cora~\cite{cora} & & - & - & - & - & - & - & $12\pm1.5$ &  $29\pm2.7$  & $53\pm3.6$   & $34\pm9.4$ & $34\pm9.5$  & \textbf{$\textbf{65}\pm3.1$}   \\ \hline 
Cora~\cite{cora} & class & - & - & - & - & - & - & $35\pm16$ &  $45\pm12$  & $72\pm12$   &   $71\pm16$ & $60\pm21$  & $\textbf{85}\pm6.5$  \\  \hline
Douban~\cite{Douban} & online-offline & - & - & - & - & - & - & $0.83$ &  $0.93$  & $2.4$  &   $0.8$ & $0.8$  & $\textbf{3.1}$ \\ 
\end{tabular}
\label{tab:n2n}
\end{table}

==> sections/Tabels/TAB_minnesota0.4patch.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|l|l|l|l|l|l|l}
         & accuracy & MAP      & AUC      & Hit      & precision\_5 & precision\_10 & time     \\ \hline
IsoRank  & 0.00               & 0.01 & 0.51 & 0.51 & 0.00         & 0.01          & 32.18  \\ \hline
BigAlign & 0.57               & 0.04 & 0.91 & 0.91 & 0.05         & 0.10          & 0.04   \\ \hline
FINAL    & 0.01               & 0.01 & 0.52 & 0.52 & 0.00         & 0.01          & 10.21  \\ \hline
REGAL    & 0.85               & 0.87 & 1.00 & 1.00 & 0.94         & 0.97          & 7.08   \\ \hline \hline
fmW      & 0.83               & 0.88 & 1.00 & 1.00 & 0.93         & 0.96          & 4.03   \\ \hline
fmW+ZM  & 0.85               & 0.89 & 1.00 & 1.00 & 0.94         & 0.97          & 1.71   \\ \hline
GRASP    & 0.25               & 0.18 & 0.93 & 0.93 & 0.27         & 0.42          & 648.43 \\ \hline
gt       & 0.90               & 0.94 & 1.00 & 1.00 & 0.98         & 0.99          & 1.24   \\ \hline \hline
PALE     & 0.93               & 0.70 & 1.00 & 1.00 & 0.90         & 0.96          & 308.98 \\ \hline
\end{tabular}
\caption{Minnesota 0.4 patch}
\label{tab:minnesota0.4patch}
\end{table}

==> sections/Tabels/TAB_n2n.tex <==
\begin{table}[h]
% \hspace{-0,4cm}
\setlength{\tabcolsep}{3.4pt}
\centering
\scriptsize
\caption{Comparison of the Mean Average Precision of different graph matching methods. We use $k=50$ eigenfunctions for the functional map representation. {We also report the percentage of eigenfunctions used w.r.t. the number of nodes of the full graph ($k\%$).}}
\begin{tabular}{l|c c|c c c c c c c c}
 & Partiality & $k \%$ & IsoRank & FINAL & REGAL & PALE & GRASP & FM$_{W}$ & FM$_{W}+$ZM & $GT$ \\ \hline
Cat & \multirow{3}{*}{patch} & 0.5 & $0.1\pm0.0$ &     $0.2\pm0.0$    &  \textbf{$\textbf{93}\pm1.9$} & $6.8\pm0.4$ & $11\pm0.0$& $68\pm14$ & $69\pm14$  & $92\pm3.9$ \\ 
Minnesota & & 1.9 &  $0.2\pm0.1$ &    $1\pm0.0$ & $87\pm3.3$ &  $13\pm0.4$  & $18\pm2$ &   $88\pm4$ & $89\pm3.7$  & \textbf{$\textbf{94}\pm1.6$}  \\
Cora &  & 2 &  $0.5\pm0.0$ &    $0.6\pm0.0$ & $54\pm3.5$ &  $22\pm2.9$  & $6.8\pm1.8$ &   $33\pm9.4$ & $34\pm9.5$  & \textbf{$\textbf{65}\pm3.1$}  \\ \hline 
Cora & class & 2 & $0.4\pm0.0$ &    $0.4\pm0.0$ & $55\pm3.4$ &  $17\pm2$  & $51\pm22$ &   $71\pm16$ & $60\pm21$  & $\textbf{85}\pm6.5$  \\  \hline
Douban  & online-offline  & 1.3 &  $0.6$ &    $1.1$ & $\textbf{70}$ &  $6$  & $0.7$ &   $0.8$ & $0.8$  & $3.1$ \\ 
\end{tabular}
\label{tab:n2n}
\end{table}

==> sections/Tabels/TAB_n2n_eigs.tex <==
\begin{table}[h]
% \hspace{-0,4cm}
\setlength{\tabcolsep}{2.7pt}
\centering
\scriptsize
\caption{MAP(\%) of the correspondence on different datasets at increasing number of eigenvectors (expressed as percentages, growing from $1\%$ to $75\%$). The correspondences are obtained from ground-truth functional maps.}
\begin{tabular}{l|C{0.9cm} |c c c c c c c}
 & Partiality & 1\% & 3\% & 5\% & 10\% & 30\% & 50\% & 75\%\\ \hline
Cat & \multirow{3}{*}{patch} & $ 86.97\pm4.92$  & $97.65\pm0.93$  &  $99.23\pm0.41$ & $99.98\pm0$  & $\textbf{100}\pm0$ & $\textbf{100}\pm0$ & $\textbf{100}\pm0$  \\ 
Minnesota & & $70.77\pm4.54$  & $90.05\pm1.97$  &  $94.42\pm1.22$ & $97.78\pm0.46$  & $99.62\pm0.1$  &  $99.98\pm0$ & $\textbf{100}\pm0$   \\
CORA & & $ 49\pm4.51$  & $68.41\pm3.5$  &  $76.22\pm2.67$ & $84.28\pm0.96$  & $93.15\pm0.56$  &  $99\pm0.18$ & $\textbf{99.54}\pm0.12$  \\ \hline 
CORA & class & $71.35\pm9.24$  & $86.87\pm3.71$  &  $90.18\pm2.65$ & $93.57\pm1.16$  & $95.96\pm0.33$  &  $99.08\pm0$ & $\textbf{99.5}\pm0$   \\  \hline
Douban   & online-offline & $1.6$  & $4.23$  &  $8.3$ & $19.91$  & $64.46$  &  $96.33$ & $\textbf{98.97}$ \\ 
\end{tabular}
\label{tab:n2n_eigs}
\end{table}

==> sections/Tabels/TAB_results.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|l|l|l|l|l|l|l}
         & accuracy & MAP      & AUC      & Hit      & precision\_5 & precision\_10 & time     \\ \hline
IsoRank  &          &     &     &     &             &              &      \\ \hline
BigAlign    &          &     &     &     &             &              &      \\ \hline
FINAL    &          &     &     &     &             &              &      \\ \hline
REGAL &          &     &     &     &             &              &      \\ \hline \hline
fmW      &          &     &     &     &             &              &      \\ \hline
fmW+ZM   &          &     &     &     &             &              &      \\ \hline
GrASP      &          &     &     &     &             &              &      \\ \hline
gt       &          &     &     &     &             &              &      \\ \hline \hline
PALE        &          &     &     &     &             &              &      \\ \hline
IONE?        &          &     &     &     &             &              &      \\ \hline
\end{tabular}
\caption{TAB}
\label{tab:tabres}
\end{table}

==> sections/Tabels/TAB_sub_perc.tex <==
% \begin{table}[h]
% % \hspace{-0,4cm}
% \setlength{\tabcolsep}{2.7pt}
% \centering
% \tiny
% \caption{MAP(\%) of the correspondence on different datasets at decreasing size of the sub graph (expressed as percentages, growing from $90\%$ to $50\%$). The correspondences are obtained from ground-truth functional maps.}
% \begin{tabular}{l|c c c c c | c c c c c}
%  & \multicolumn{5}{c}{patch} & \multicolumn{5}{c}{holes} \\
%  & 90\% & 80\% & 70\% & 60\% & 50\%  & 90\% & 80\% & 70\% & 60\% & 50\%\\ \hline
% Minnesota & $95.82\pm1.84$ & $96\pm1.98$ & $94.47\pm1.9$ & $94\pm1.6$ & $94.12\pm1.27$ & $68.19\pm1.91$ & $50.36\pm4.11$ & $46.28\pm3.5$ & $51.7\pm3.0$ & $53.80\pm3.3$\\
% CORA~\cite{cora} & $82.67\pm2.4$ &  $74.45\pm2.27$ & $67.2\pm2.56$ & $65\pm3.1$ & $60.03\pm2.45$ & $70\pm3.58$ & $55.52\pm4.16$ & $45.59\pm2.67$ & $41.87\pm2.3$ & $38.08\pm2.9$\\  
% Citeseer~\cite{cora} & $83.12\pm1.88$ & $77.68\pm3.48$ & $71.33\pm4.48$ & $68.5\pm3.13$ & $65.41\pm5.21$  & $74.8\pm2.83$  & $62.4\pm2.7$ & $ 54.97\pm2.47$ & $51.07\pm3.21$ & $48.87\pm2.8$  \\  \hline
% \end{tabular}
% \label{tab:n2n_subs}
% \end{table}

%%%
\begin{table}[h]
% \hspace{-0,4cm}
\setlength{\tabcolsep}{2.7pt}
\centering
\tiny
\caption{MAP(\%) of the correspondence on different datasets at decreasing size of the sub graph (expressed as percentages, decreasing from $90\%$ to $50\%$) with two type of partiality: patch (first table) and holes (second table). The correspondences are obtained from ground-truth functional maps.}
\begin{tabular}{l|c c c c c }
% & \multicolumn{5}{c}{patch} \\
\textbf{patch} & 90\% & 80\% & 70\% & 60\% & 50\% \\ \hline
Minnesota & $95.82\pm1.84$ & $96.00\pm1.98$ & $94.47\pm1.90$ & $94.00\pm1.60$ & $94.12\pm1.27$ \\
CORA & $82.67\pm2.40$ &  $74.45\pm2.27$ & $67.20\pm2.56$ & $65.00\pm3.10$ & $60.03\pm2.45$ \\  
Citeseer & $83.12\pm1.88$ & $77.68\pm3.48$ & $71.33\pm4.48$ & $68.50\pm3.13$ & $65.41\pm5.21$  \\  \hline
\end{tabular}
\bigskip

\begin{tabular}{l|c c c c c }
% & \multicolumn{5}{c}{holes} \\
\textbf{holes} & 90\% & 80\% & 70\% & 60\% & 50\%  \\ \hline
Minnesota & $68.19\pm1.91$ & $50.36\pm4.11$ & $46.28\pm3.5$ & $51.70\pm3.00$ & $53.80\pm3.30$\\
CORA & $70.00\pm3.58$ & $55.52\pm4.16$ & $45.59\pm2.67$ & $41.87\pm2.30$ & $38.08\pm2.90$\\  
Citeseer & $74.80\pm2.83$  & $62.4\pm2.70$ & $ 54.97\pm2.47$ & $51.07\pm3.21$ & $48.87\pm2.80$  \\  \hline
\end{tabular}
\label{tab:n2n_subs}
\end{table}



==> sections/Tabels/TAB_time.tex <==
\begin{table}[h]
% \hspace{-0,4cm}
\setlength{\tabcolsep}{2.0pt}
\centering
\tiny
\caption{Comparison of the computational time (in seconds) needed by different methods to compute a node-to-node correspondence, across several datasets. Spectral based methods (last two columns) are the most efficient.}
\begin{tabular}{l|C{0.8cm} |c c c c c c c}
 & Partiality & IsoRank & FINAL & REGAL & PALE & GRASP & FM$_{W}$ & FM$_{W}+$ZM \\ \hline
Cat & \multirow{3}{*}{patch} & $270.44\pm9.84$  & $156.49\pm2.73$  &  $36.78\pm0.86$ & $3586.4\pm109.5$  & $1057.7\pm100.59$ & $\mathbf{20.73}\pm1.67$ &$\mathbf{5.45}\pm0.28$ \\  % $79.56\pm2.77$ &$64.28\pm0.89$  &$58.83\pm1.17$  \\ 
Minnesota & &  $32.18\pm3.94$ &   $10.21\pm0.15$  & $7.08\pm0.07$  & $145.72\pm9.14$ & $648.43\pm267.5$  &   $\mathbf{2.83}\pm0.66$  & $\mathbf{0.33}\pm0.03$   \\ % $4.03\pm0.96$  & $1.71\pm0.33$   & $1.24\pm0.3$   \\
Cora & &  $31.54\pm3.1$ &    $10.48\pm0.55$ & $7.33\pm0.15$ &  $211.99\pm1.87$  & $198.22\pm148.3$ &   $\mathbf{2.89}\pm0.42$ & $\mathbf{0.39}\pm0.4$\\ \hline  % $4.12\pm0.47$ & $1.62\pm0.1$  & \textbf{$\textbf{1.23}\pm0.05$}  \\ \hline 
Cora & class & $14.92\pm2.4$  &    $51.61\pm10.2$ & $10.92\pm0.9$  & $434.13\pm35.6$  & $118.61\pm72$  & $\mathbf{1.96}\pm0.1$  & $\mathbf{0.38}\pm0.02$\\  \hline % $3.42\pm0.37$  & $1.84\pm0.25$   &$1.46\pm0.27$  \\  \hline
Douban   & online-offline &  $11.54$  &    $27.07$  & $10.41$  & $337.56$   & $16.32$  &  $\mathbf{4.43}$ &$\mathbf{0.03}$  \\ % $8.80$ &$4.44$  & $4.37$ \\ 
\end{tabular}
\label{tab:n2n_time}
\end{table}

% \begin{table}[h]
% \centering
% \caption{Comparison of the Computation Time (in seconds) of the correspondence computed on different graphs by different methods.}
% \begin{tabular}{l|c|c c c c c c c c}
%  & Partiality & IsoRank & FINAL & REGAL & PALE & GRASP & FM$_{W}$ & FM$_{W}+$ZM & $GT$ \\ \hline
% Cat\cite{shrec2016} & \multirow{3}{*}{patch} & $0\pm0$  & $0\pm0$  &  $0\pm0$ & $0\pm0$  & $0\pm0$ & $0\pm0$ &$0\pm0$  &$0\pm0$  \\ 
% Minnesota & &  $32.18\pm3.94$ &   $10.21\pm0.15$  & $7.08\pm0.07$  & $145.72\pm9.14$ & $648.43\pm267.5$  &   $2.83\pm0.66$  & $0.33\pm0.03$   & $0.0$   \\ 
% Cora\cite{cora} & &  $31.54\pm3.1$ &    $10.48\pm0.55$ & $7.33\pm0.15$ &  $211.99\pm1.87$  & $198.22\pm148.3$ &   $2.89\pm0.42$ & $0.39\pm0.4$  & $0.0$  \\ \hline  
% Cora\cite{cora} & class & $14.92\pm2.4$  &    $51.61\pm10.2$ & $10.92\pm0.9$  & $434.13\pm35.6$  & $118.61\pm72$  & $1.96\pm0.1$  & $0.38\pm0.02$   &$0.0$  \\  \hline 
% Douban\cite{Douban}   & online-offline &  $11.54$  &    $27.07$  & $10.41$  & $337.56$   & $16.32$  &  $4.43$ &$0.03$  & $0.0$ \\ 
% \end{tabular}
% \label{tab:n2n_time}
% \end{table}

==> sections/fig_partial.tex <==
\begin{figure}[t]
\vspace{0.2cm}
\centering
\begin{subfigure}[b]{0.48\textwidth}
\centering
\begin{overpic}
[trim=0cm 0cm 0cm 0cm,clip,width=0.999\linewidth,grid=false]{./figures/patch_C.png}
\put(1,51){\tiny Minnesota}
\put(4,33){\tiny CORA}
\put(3,15){\tiny Citeseer}
\put(20,51){\tiny $90\%$}
\put(37,51){\tiny $80\%$}
\put(53,51){\tiny $70\%$}
\put(70,51){\tiny $60\%$}
\put(87,51){\tiny $50\%$}
\end{overpic}
\caption{\label{fig:patch} Patch}

\end{subfigure}
 \hfill
 \begin{subfigure}[b]{0.48\textwidth}
\centering
\begin{overpic}
[trim=0cm 0cm 0cm 0cm,clip,width=0.999\linewidth]{./figures/holes_C.png}
\put(1,51){\tiny Minnesota}
\put(4,33){\tiny CORA}
\put(3,15){\tiny Citeseer}
\put(20,51){\tiny $90\%$}
\put(37,51){\tiny $80\%$}
\put(53,51){\tiny $70\%$}
\put(70,51){\tiny $60\%$}
\put(87,51){\tiny $50\%$}
\end{overpic}
\caption{\label{fig:holes} Holes}
\end{subfigure}
 \hfill
\caption{\label{fig:partial} Robustness of the map to the action of two partialities: patch and holes. The partialities are increasingly wider, from a subgraph with $90\%$ of the nodes to a subgraph with $50\%$ of the nodes. As partiality increases, the functional map structure becomes less defined.}
\end{figure}


==> sections/fmapGraph.tex <==
\section{\label{sec:method}Spectral maps for subgraphs}



In this work, we consider the setting where we are given a graph $\Gg$ and a possibly noisy subgraph $\Gs = (\Vs,\Es)$ of $\Gg$, such that $\Vs \subseteq \Vg$ and $\Es \subseteq \Eg$. %As done for $\Gg$, we define the adjacency matrix $\As$ and the Laplacian $\Laps$. % of $\Gs$.
%
When moving from surfaces to graphs, Equation~\ref{eq:fmap} takes a simpler expression as we show in Appendix~\ref{sec:matrint}.

==> sections/method.tex <==
\section{\label{sec:method}Spectral maps for subgraphs}



==> sections/results.tex <==
\section{Empirical results and analysis}
\label{sec:results}
In this section we validate the claims made in the previous sections with additional qualitative and numerical results. More experiments and details of the used datasets can be found in Appendix~\ref{sec:exp_details}.


\input{sections/Figs/robust_rewire}
\subsection{\label{sec:rob_rewire_exp}Robustness to rewiring}
%
In section \ref{sec:RobRewire}, we claimed that the functional representation is robust to changes in graph connectivity. 
{%In our setting, for a map representation to be robust
For this to be true, we expect that small changes in graph connectivity lead to small changes in the matrix coefficients. See Appendix \ref{app:rob_rewire} for the formal definition.}

{In Figure~\ref{fig:robustRewiring}, we evaluate the changes of the functional map at increasing percentages of rewiring of a subgraph.
We consider six graphs and compute a subgraph from each one. Then, we apply small incremental changes to the topology of the subgraphs, with increments of $3\%$ of the total number of edges; the changes are performed by removing and adding random edges, obtaining new subgraphs $G_i$.
The plot on the right shows how much the functional map representation is affected by the increasing topological changes compared to adding Gaussian noise. In all the cases, the rewiring produces less variation in the functional map than adding Gaussian noise. In particular, the functional representation is more robust on larger graphs, such as cat (10000 nodes) or citeseer (2120 nodes), while on smaller graphs such as QM9 (29 nodes) and Karate (34 nodes), removing or adding an edge has a more significant impact. 
This observation demonstrates the effectiveness of the spectral representation, especially on larger graphs.
In Appendix \ref{app:rob_rewire}, we show the complete qualitative analysis; while in Appendix \ref{sec:add_rewire} we push this experiment to stronger rewiring.
}
% In Figure~\ref{fig:robustRewiring}, we test this behavior on different graphs. 
% In each row, we select a graph $\Gg$ (pictured in the first column) and compute a subgraph $\Gs$ from it (second column). Then, we apply small incremental changes to the topology of the subgraphs, with increments of $3\%$ of the total number of edges; the changes are performed by removing and adding random edges, obtaining new subgraphs $G_i$. 
% In the figure, in the second column we plot one representative example (per dataset) of such topological modifications, depicting the added edges in green, and the removed edges in red. 
% The matrices appearing in the figure show the element-wise perturbation of the functional map matrix between $\Gg$ and $\Gs$ after performing the rewiring operations.
% {From these experiments, we observe that a little change in the graph connectivity induces a small change in the functional map coefficients. In particular, the error initially accumulates on a specific region of the map and then spreads, gradually losing its sparse structure.} %as the eigenspaces defined by the first eigenvectors of the two graphs gradually get more.}

\subsection{Signal transfer}
% \begin{figure}[h!]
% % \vspace{0.0cm}
% \centering
% \begin{overpic}
% [trim=0cm 0cm 0cm 0cm,clip,width=0.8\linewidth]{./figures/func_transf_cut.png}
% \put(10,1){\footnotesize {$f: \Gg \rightarrow \mathbb{R}$}}
% \put(48,1){\footnotesize {$\hat{g}: \Gs \rightarrow \mathbb{R}$}}
% \put(77,1){\footnotesize {$(g-\hat{g})^2$}}
% \put(27,26){\footnotesize {$C=$}}
% \put(31,13){\Huge $\longrightarrow$}
% \put(97.4,25){\tiny $1$}
% \put(97.4,18.5){\tiny $0$}
% \put(-4,18){\tiny $min(f)$}
% \put(-4,24.5){\tiny $max(f)$}
% \end{overpic}
% \caption{\label{fig:signTransfer} Illustrative example of a signal transferred from the graph $\Gg$ (left) to the sub-graph $\Gs$ (right) using the functional map matrix $C$ (top). The rightmost graph reports the node-wise squared difference between the original and the reconstructed signal.}
% \end{figure}
Within a graph, nodes may often come with numerical or vector-valued attributes, for instance, encoding molecular properties in PPIs, user identities in social networks, or positional encodings to better distinguish and characterize nodes. We can model such data as a collection of functions $f: \Vg \rightarrow \mathbb{R}$ that map each node of $\Gg$ to a real value. 
{Recent works \citep{PE_rewiring} have demonstrated that transferring the positional encoding from a graph to its rewired version can improve GNN performance.}
The functional map $C$ allows us to transfer these functions from a graph $\Gg$ to a subgraph $\Gs$ without requiring the explicit computation of a node-to-node correspondence. 
For each function $f$, it is sufficient to project $f$ onto the Laplacian eigenfunctions of $\Gg$, apply the linear transformation $C$ to the obtained coefficients, and finally reconstruct the signal on the target graph $\Gs$ as a linear combination of its Laplacian eigenfunctions. The described procedure is implemented by the simple formula: 
%
\begin{align}
\hat{g} = \EVECs C \EVECg^\top f \,,
\label{eq:transfer}
\end{align}
{where the function $\hat{g}: \Vs \rightarrow \mathbb{R}$ is the transfer of $f$ to $\Gs$.}
%
%This formulation allows us to define a correspondence between graphs even when a node-to-node correspondence is not well defined. See Supplementary Material for further details and examples on this aspect.
%In Table\ref{tab:func_transfer},
Motivated by the results from \cite{PE_rewiring}, we leverage this property of the spectral representation to transfer the positional encoding computed on a graph to its subgraphs. 
% Given a signal $f$ defined over $\Gg$ (left), we transfer $f$ to the subgraph $\Gs$ (middle) through the functional map $C$ (top), obtaining a new signal $\hat{g} : \Gs \rightarrow \mathbb{R}$. 
% To evaluate the fidelity of the transferred signal, we compute the root mean squared error between the transferred signal $\hat{g}$ and the ground truth signal $g$ (obtained via the ground truth node-to-node correspondence) through the formula: $\frac{\sum_{i=1}^{n} (\hat{g}_i - g_i)^2}{n (max(f)-min(f))}$.
% In Table~\ref{tab:func_transfer}, we report a similar experiment on graphs from different datasets. We consider pairs composed by the original graph and a series of subgraphs extracted according to a semantic criterion, e.g., nodes belonging to the same class or nodes connected by the same type of edge. On each pair we transfer the signal defined over the original graph to the subgraph using a functional map represented in the first 50 eigenfunctions. The last column reports the average reconstruction error. %\textcolor{red}{Luca: è un po' difficile interpretare i risultati i tabella.}
%{The signal transfer achieves the best performance when the signal is continuous. This is due to the use of the first few Laplacian eigenvectors, which are provably optimal for representing smooth signals~\cite{Aflalo15}. %that act as a low-pass filtering of the signal, removing high frequency noise.
%On FraudAmazon, Amazon Photo and Amazon Computer larger errors may be due to both the discrete and sparse features, and the bigger size of the graphs. Since we use a fixed amount of eigenvectors in our experiments (50), that is a small percentage with respect to graph size (see column $k \%$), it is harder to represent discrete signals on these graphs. In Figure 3 of the supplementary material, we show how increasing the number of eigenvectors effectively reduces the error.}
{In Figure~\ref{fig:func_transfer}, we analyze the functional map transfer performance while increasing the number of eigenfunctions used for the map representation. %We evaluate the fidelity of the transferred signal with the Root Mean Squared Error between the transferred signal $\hat{g}$ and the ground truth signal $g$ (obtained via the ground truth node-to-node correspondence).
% \begin{equation}
%     NRMSE = \frac{\sqrt{\frac{1}{n}{\sum^n_{i}{(g(i)-\hat{g}(i))^2}}}}{\overline{g}}
% \end{equation}
% where $n$ is the number of nodes in the subgraph and $\overline{g}$ is the mean of the signal $g$. 
We consider pairs composed of the original graph and a series of subgraphs extracted according to a semantic criterion, e.g., nodes belonging to the same class or nodes connected by the same edge type. We transfer the Random Walk Positional Encoding \citep{rwPE} computed on the full graphs to the subgraphs. We normalize each dimension of the node features of the original graph to exhibit zero mean and unitary standard deviation throughout all the nodes, and then transfer this signal through Equation \ref{eq:transfer}.
In Figure~\ref{fig:func_transfer}, we can see how the Root Mean Squared Error between the functional map and the ground truth transfer (we refer to Appendix \ref{app:sig_transf} for more details on the evaluation) decreases as the number of eigenfunctions increases. 
In particular, the error rapidly decreases at 10\%-30\% of eigenvectors. 
This behavior demonstrates that using a compact representation with few eigenvectors can approximate the signal well. 
The qualitative examples on the left of Figure \ref{fig:func_transfer} portray the transferred signal on PPI0. Already at 1\% of the eigenfunctions the transfer reaches a good approximation, while at 75\% it is almost identical. 
In Appendix \ref{sec:nume_eig}, we show more experiments with different number of eigenfunctions.}
\input{sections/Tabels/TAB_transfer}

{Suppose the graph and subgraphs are equipped with features independent of topological changes (like in Citeseer). In that case, we can compute the functional map $C$ from these features without needing ground truth correspondence a priori. To show the effectiveness of this alternative, in Appendix~\ref{app:sig_transf}, we show the results of signal transfer via an estimated $C$.}

\subsection{Node-to-node correspondence}
\input{sections/Tabels/TAB_n2n}

One of the advantages of the spectral representation is to reduce the NP-hard problem of finding node-to-node correspondences (usually formulated as a quadratic assignment problem~\citep{qap}) to the more tractable (polynomial) problem of finding the linear transformation between the reduced eigenbases of the graphs (at least under the reasonable assumption of smoothness of the sought correspondence, i.e., nearby nodes on the input graph are located nearby also on the target subgraph). {Assuming a list of $m$ corresponding functions staked column-wise in two matrices $F_1 =\{f_1^{(1)} | \dots | f_1^{(m)}\}$ and $F_2 = \{f_2^{(1)} | \dots | f_2^{(m)}\}$, respectively defined on the node sets $\Vg$ and $\Vs$, the general functional map matching algorithm corresponds to the following minimization problem:
\begin{equation}
\label{eq:fmap_opt1}
    \argmin_C \| C \Phi_1^\top F_1 - \Phi_2^\top F_2 \|_2^2 + reg(C) \quad,
\end{equation}
where $reg(C)$ is a regularization imposing desired properties on $C$ (e.g. sparsity, diagonal structure). The corresponding functions can be any consistent function between the two graphs, such as input features coming with the data.} %Finally, the functional map is converted into a node-to-node correspondence between the two input graphs by transferring indicator functions or with more advanced refinement techniques ~\citep{melzi2019zoomout}.}

In this experiment, we apply two functional map-based matching algorithms.
%to recover such linear transformation. 
We adopt the off-the-shelf partial functional map algorithm ($FM_W$) \citep{rodola2017partial} and then the ZoomOut refinement~\citep{melzi2019zoomout} ($FM_W+ZM$). We compare the spectral representation with the network alignment methods proposed in the benchmark \citep{NetAlignBencharmk}: IsoRank~\citep{IsoRank}, FINAL~\citep{FINAL}, REGAL~\citep{REGAL} and PALE~\citep{PALE}.
For all the methods, we use as input 50 landmark matches. For the two functional map methods we truncate the basis to the first 50 eigenvectors and use smooth indicator functions computed on the given landmarks as corresponding functions. We refer to the appendix \ref{sec:n2n_details} for further details.

To investigate the degradation of the correspondence induced by the truncated eigenbasis, excluding errors generated by the matching algorithm, we also compute the correspondence starting from the ground-truth functional map (GT in the table).
%
%With this experiment we test the ability of the functional representation to encode a node-to-node correspondence. %We consider both the cases in which the ground truth functional $C_{GT}$ map is given, and the case in which the  
% In Table\ref{tab:n2n}, we test how well a functional map can encode such correspondences. We consider both the ground truth functional map $C_{GT}$ and both the   functional map computed with the partial functional map framework $fmW$ and the ZoomOut\cite{melzi2019zoomout} refinement $fmW+ZM$. We refer to the supplementary material for the implementation details.
%

We report in Table~\ref{tab:n2n} the Mean Average Precision (MAP) defined as $\frac{1}{n} \sum_{i=1}^{n} \frac{1}{ra_i}$ where $ra_i$ is the rank (position) of positive matching node in the sequence of sorted candidates.
%\textcolor{red}{Commentare risultati in tabella qui di seguito.}
For our evaluation we consider different graphs and subgraphs. 
We extract 10 partial graphs by considering k-hops subgraphs starting from random points.
% We perform a similar extraction also on Minnesota and CORA. 
As we can see from the $GT$ column, the functional representation seems to  preserve well the correspondence on these graphs, reaching the highest performance in almost all cases. 
{Even if the functional map based methods leverage a more compact representation, their performance is satisfactory, being the best performing method in Minnesota and the second best in the other two datasets. Moreover, Appendix \ref{app:compTime} demonstrates that the functional map representation remains the fastest method in every graph.}
% Also the  performance of the functional map based methods is satisfactory, being the best performing method in Minnesota and the second best in the other two datasets.
%The functional map seems to perform particularly well on the Minnesota graph. This is probably because it represents an example of planar graph, where an almost regular structure can be defined. 
%
We note that for social graphs like CORA,   characterized by few nodes with high degrees, the performance improves when the subgraph is semantically meaningful, obtained by removing all the nodes belonging to a specific class (fourth row).
{REGAL performs better since it is an ad-hoc algorithm for node-to-node correspondences on graphs, while our method is a more general solution that leverages a simple linear system. We find it remarkable that using a functional map as a representation without any fine-tuning works better in most cases, %We also want to note that 
%The objective of this experiment is to introduce a spectral representation as a better representation to handle correspondences and not to provide a state-of-the-art graph matching algorithm. We are optimistic that
and are positive that this could lead to follow-up work for subgraph matching.}

Finally, we test the functional representation on Douban~\citep{Douban}, a real-world dataset composed of an online and offline version of the same social network. In this case, both the nodes and connectivity are very different between the two graphs, resulting in incompatible eigenbases making this scenario particularly challenging for a functional representation, as can also been observed by the low accuracy achieved using the $GT$ functional map.
%
{In Appendix~\ref{sec:add_exp} and \ref{sec:nume_eig}, we further investigate the performance of the functional representation at increasing partiality and number of eigenfunctions.}

%In the supplementary material we further analyze the difference between Mesh Laplacian (with Neumann boundary conditions) and Normalized Graph Laplacian.



==> sections/supmat.tex <==
\section{Supplementary}

\textbf{Figure}: functional map between full cat and partial (cut and holes), both with mesh laplacian (Neumann) and normalized graph laplacian. Mask computed from eigenvalues \\
\textbf{Message}: On cut, the C are very similar. Surprisingly with the normalized graph laplacian the C is even sharper. This translates to better performance on the point-to-point correspondence retrieval from the C, see results section on cat 0.4 patch\_mesh 
The mask becomes more different on hole partiality. In the supplementary, I could add a table with the accuracy and other numeric evaluations of Fm with the different laplacian.

\textbf{Figure}:
{(sketch) C maps computed with different laplacian. On the left there are the maps computed with mesh laplacian (Neumann condition) and normalized graph laplacian, respectively. They are both computed on a partial mesh obtained cutting half cat. On the right a partiality given by holes}
 
 \textit{(Supplementary?)} \textbf{Figure}: full spectrum and eigenvector on karate\\ 
\textbf{Message}: Show eigenvalues with high multiplicity due to inner simmetries  

\textbf{Choice of the Laplacian} Compare different Laplacians and the structures that emerge from the functional map matrix, to motivate our choice. Note that the normalized graph Laplacian assumes that we do not have graphs with isolated nodes.

\textbf{PFM} Rodol\`{a} and colleagues~\cite{rodola2017partial} extended the functional maps framework to the case where $\N$ is a partial shape and rewrite the minimization from equation ~\ref{eq:fmap} as follows: 
\begin{align}
\label{eq:partialfmap}
     C = \underset{C \in \mathbb{R}^{k \times k}}{\arg\min} \| CF - B(\eta(\nu)) \|_{2,1} + \rho_{part}(\nu) + \rho_{corr}(C) .
\end{align}
Here we briefly describe the modifications that are relevant to our method and refer to ~\cite{rodola2017partial} for all the details.
The minimization is not only on $C$ but also on $\nu$, an indicator function representing the surface patch on $\M$ that corresponds to $\N$. We do not consider this because we work with graphs and without surfaces. The same holds for $\rho_{part}(\nu) $.
The norm adopted for the term on the probe functions is the $L_{2,1}$ matrix norm, which promotes column-sparse matrices to improve robustness to possible outliers.
$\rho_{corr}(C)$ fosters additional structure to $C$ and is defined as: 
\begin{align}
\label{eq:regularizerC}
\rho_{corr}(C) = \mu_1 \| C \odot W \|_{2}^{2} + \mu_2 \sum_{\ell \neq h} (C^{\top}C)_{\ell,j}^2 + \mu_3 \sum_{\ell} ((C^{\top}C)_{\ell,\ell} - d_{\ell})^2n ,
\end{align}
where each term has its weight $\mu_1$, $\mu_2$ and $\mu_3$.
$W$ is a mask matrix that acts through element-wise multiplication $\circ$ and encodes the relation between the eigenvalues of the two shapes, which approximates the anted-diagonal structure of $C$ induced by the partiality. 
The term weighted by $\mu_2$ promotes orthogonality of the map by penalizing the off-diagonal entries of $C^{\top}C$.
Finally $d_{\ell} \in \{0, 1\}, \ \forall \ell$, and the ones equal to $1$ represent the singular values of $C$ that are expected to be non-zero. 

\textbf{Comparisons with GRASP?}

\subsection{Failure cases}
%
As we demonstrate empirically, this behavior is not universal across all types of graphs

\subsection{Regularizing effect} Nel main abbiamo scritto qualche volta che la C ha un regularizing effect, con il quale intendiamo che se la mappa o il segnale sono rumorosi, abbiamo low pass aggratis. Inoltre e' ben definita anche nel caso non punto-punto. Dobbiamo supportare questi claim con qualche test.
